Discrete Auto-regressive Variational Attention Models for Text Modeling

Variational autoencoders (VAEs) have been widely applied for text modeling. In practice, however, they are troubled by two challenges: information underrepresentation and posterior collapse. The former arises as only the last hidden state of LSTM encoder is transformed into the latent space, which is generally insufficient to summarize the data. The latter is a long-standing problem during the training of VAEs as the optimization is trapped to a disastrous local optimum. In this paper, we propose Discrete Auto-regressive Variational Attention Model (DAVAM) to address the challenges. Specifically, we introduce an auto-regressive variational attention approach to enrich the latent space by effectively capturing the semantic dependency from the input. We further design discrete latent space for the variational attention and mathematically show that our model is free from posterior collapse. Extensive experiments on language modeling tasks demonstrate the superiority of DAVAM against several VAE counterparts.

==> sections/bkup.tex <==
\section{Introduction}

Combined deep neural networks with an corresponding variational learning strategy, Variational Autoencoders (VAEs)~\cite{Kingma2013AutoEncodingVB} becomes one of the most representative work of latent variable models. As the  marginal likelihood $p_{\theta}(\textbf{x})$ is  intractable, it is impossible to obtain true  posterior distribution $p_{\theta}(\textbf{z}|\textbf{x})$ directly by Bayes. Instead, VAEs introduce a approximate posterior distribution $q_{\phi}(\textbf{z}|\textbf{x})$ (i.e. the $\mathit{encoder})$, and  narrow the gap between true  posterior distribution and approximate posterior distribution by maximizing the the evidence
lower bound (ELBO):\\
\begin{equation}\nonumber
\mathbb{E}_{\textbf{z} \sim q_{\phi}(\textbf{z}|\textbf{x})}[\log  p_{\theta}(\textbf{x}|\textbf{z})] - D_{KL}(q_{\phi}(\textbf{z}|\textbf{x}) \Vert p(\textbf{z})),
\end{equation}
where $p_{\theta}(\textbf{x}|\textbf{z})$ represents likelihood function to generate samples (i.e. the $\mathit{decoder}$).

However, modeling RNN-based languages model with VAEs is prone to suffer from posterior collapse and information bottleneck. The former arises from the fact training often falls into a  trivial local optimum when a strong decoder is learnt, thus decoder ignoring the latent variable and encoder failing to encode any information from data distribution. Many efforts have focused on finding solutions to solve posterior collapse including re-weighting the KL loss~\cite{Bowman2015GeneratingSF,Kingma2017ImprovedVI,Fu2019CyclicalAS}, revising the model~\cite{Yang2017ImprovedVA,Semeniuta2017AHC,Xu2018SphericalLS} and modifying the training procedure~\cite{He2019LaggingIN,Li2019ASE}. The latter results from the fact that the only last hidden state in RNN-based VAEs model has been employed and other hidden states have been ignored, where Attention-based Seq2Seq model~\cite{Bahdanau2014NeuralMT} cannot be applied into VAEs model. Currently, little effort has tried to solve this problem, as existing VAEs models adopt low-dimension latent space, 
would need to enlarge latent space into high dimensional space if required to make most of information in all hidden state, and then cause the unreliable generation no matter whether latent variables are independently identically distribution (e.g.iid) or not. When latent variables fit independently identically distribution, that is to say each latent variable would be related to one hidden state. Under the circumstance, noises are more likely to be generated instead of samples from true data distribution since a set of latent variables with causal relationship cannot not from the prior distribution. For another case where latent variables violate independently identically distribution, all latent variables would be integrated as one part where the overall latent space would be high dimensional and sparse, thus causing training procedure being unstable. These two cases will be analyzed and verified in experiment part.  

Recently, the generative model of Vector Quantised-Variational AutoEncoder (VQ-VAE)~\cite{Oord2017NeuralDR} has obtained great success in image generation, especially high quality images generated from VQ-VAE-2~\cite{Razavi2019GeneratingDH} where multi-scale hierarchical organizations of VQ-VAE are employed has obtained better Inception Score~\cite{Salimans2016ImprovedTF} and Fréchet Inception Distance (FID)~\cite{Heusel2017GANsTB} over BigGAN~\cite{Brock2018LargeSG}. VQ-VAE relaxes a static prior hypnosis in the training process, and latent variables don't need to be reparameterized by the specific prior, thus posterior collapse being avoided directly. Compared with traditional VAEs model, VQ-VAE adopts the discrete high dimensional latent space rather than the continuous low-dimension latent space, where image structure and details are able to be preserved better. 

Inspired by VQ-VAE~\cite{Oord2017NeuralDR}, in this paper, we proposed a novel generative RNN-based language model named Discrete VAE to solve posterior collapse and information bottleneck in traditional VAEs models. The problem of posterior collapse could be easily avoided as VQ-VAE due to no static prior has been employed in proposed model to restrain the latent variables during the training procedure. To address the information bottleneck effectively, we establish a fixed size of discrete codebook where records the information in latent space as the VQ-VAE, and each hidden state would be encoded into a latent variable, each latent variable would seek its nearest vector recorded in codebook, and then all latent variables would be clustered by vectors in codebook closely via optimizing, thus all hidden states information being fully utilized. With these information, attention-based Seq2Seq model could be combined into our proposed model, and then the problem of information bottleneck could be eliminated. Finally, auto-regressive model pixelCNN will be employed to learn a flexible prior (pixelCNN prior) after trainging procedure, then long sequence could be well-generated with the prior.

% There are some differences between high-dimension discrete latent space and high-dimension continuous space, where both models could fully use the information. For the one case where latent variables in continuous space fix independently identically distribution, only a set of independent latent variables where causal relations between latent variables are ignored could be sampled from the static prior, while proposed model could deploy pixelCNN prior to sample a set of causal latent variables. Compared with another case where latent variables in continuous space violate independently identically distribution, our model deploys a set of latent variables to represent a sentence, and seek nearest vector in the codebook for each latent variable instead of integrating all latent variables into overall part. Under this circumstance, our latent space for each latent variable won't suffer from the problem of sparsity as each latent variable could be in a low-dimension space although space for a set of latent variables would be extremely high dimensional; Also, all variables are clustered closely by discrete vectors in the codebook, which enable every discrete vector contains the semantic information. With the combination of a series of discrete vectors, it would be equipped with strong capacity of expressing the any causal relationship for generating a sentence.

Our contributions can thus be summarised as:
\begin{enumerate}
\item Our work mainly focused on the solution to the information bottleneck in RNN-base language generative model of VAEs, and testify that only latent variables in discrete space could be combined with attention-based Seq2Seq models properly and find the solution for this problem.
\item Our work incorporates the VQ-VAE model into the language generative model, relaxes the static prior assumption in the training process, deploys the pixelCNN network to generate more flexible prior, where enable the posterior collapse to be avoided directly.
\item our work deploys the pixelCNN prior to sample a set of latent variables with causal relationships from the codebook where each vector has the strong semantic information, thus generating a sentence with strong logical relationship.
\end{enumerate}

\fang{Seq2Seq model~\cite{Sutskever2014SequenceTS}}
\fang{Auto-regressive model: PixelCNN~\cite{Oord2016PixelRN}}
\fang{PixelCNN++~\cite{Salimans2017PixelCNNIT}}
\fang{GatedPixelCNN~\cite{Oord2016ConditionalIG}}
\fang{WaveNet~\cite{Oord2016WaveNetAG}}







\begin{table*}[h]
\begin{center}
\label{tab:generated_sentences}
\footnotesize
\begin{tabular}{l|l}
\toprule
Method & Samples \\\hline
pretrain- &  
%does anybody know who 's one like them?? please help me! [/s] \\
\tabitem why do they think boys are \_UNK in wrestling? \_UNK is in first \_UNK with no scholarship to them [/s]\\
%FBP($\lambda$=8)-&
%VAE & what would you do for birds \_UNK day? feast day:) go on the beaches with a \_UNK!:) [/s]\\
%&is troy hogan really fat? if so, who is her guy? depends on who their at home, she's fast and more of a band. [/s]\\
%&also giants has a reputation in the colts who can play them? i think it will win looking through a rod a team. [/s]\\
%&what happens if a child is a rich woman? the union will be done as a \_UNK. [/s]\\
FBP($\lambda$=8)-& \tabitem where is it that morning when snow on thanksgiving ? what's the next weekend ? dress it!!!! my mother was \\
VAE&the teen mom and i love her and she just is going to be my show. [/s]\\ 
%&why do i fall asleep at my feet? i play really loud, but it well hurts any other \_UNK. thats not quite. coz in an \\
%&warm up it is not \_UNK! you are describing dreams. [/s]\\
%&how can i train a lot to train \_UNK? i really need equipment. take the range on your muscles and enter the walls,\\ 
%&slowly interact with the air and will accelerate through. [/s]\\
%&would you like to go to iraq how many were them and how they made the country? given it to the \_UNK if \\
%&earth war. the only way we knew it is, our mind without controlling our oil. [/s]\\
%&why are neocons coming to house!!!!!!!!!?they are horrible when they are a kid and every religion really \\
%& does n't get;15\% nobody should say it is nice to come to the party and take care of them it happened on the same \\
%&road they had an idea about this... [/s]\\
&\tabitem are they allowed to join ( francisco ) in \_UNK. giants in the first place.? check out other answers. do you miss \\
& the economy and not taking risks in the merchant form, what would you tell? go to the yahoo home page and ask \\
& what restaurants follow this one. [/s]\\
%&where can i go to get really good reasons? for example, located in the atlanta sky, chicago, california. where \\
%&have i got a clue where i have been watching... [/s]\\ 
\hline
GVAM 
%& does u have a \_UNK to find an essay there list that's there more authentic!! [/s]\\
& \tabitem what is it lyrics when your rich [/s]\\
&if you find a from the state from the political flags, you get the farm library. [/s]\\
%&why do you have to tell boy. i should tell you that should tell boy. i need? then and others? then is the best [/s]\\
%&do the who who have a in need the child and what is the one cat cat that the one knows of the child of cat [/s]\\
& \tabitem will women... as melting for...? as the best national i'm robbed to a condition mate montreal for a condition \\
& and out for you you know. [/s]\\
\hline
% DVAM &  what is the best way to get rid of high blood pressure in bed in \_UNK? [/s]\\
%  & where to a good one that can help me to the new york state? try \_UNK. [/s]\\
%  & is the guy who 's an alcoholic beverage killer? no. his wife and they do n't. [/s]\\
%  & where a best? many places you can get more information from a reliable site to learn japanese. [/s]\\
 DVAM & \tabitem i need to start a modeling company ! any suggestions on what is a reliable topic? [/s]\\
%  & is i only attracted tp 1 person without the consent of my wife or her husbands with her permission? it's all\\
%  & about your maturity level. [/s]\\
 & \tabitem does anyone agree, there is a global warming of the earth? in general. there are several billion things, including \\
 &the earth, solar system. [/s]\\
% & do my name the band name has a song? it goes to “the blues brothers”, it's a song i heard of it. [/s]\\ 
% & can their people just \_UNK themselves? is it worth an effort to lose weight? i am not sure but if you were to take\\
% &those, i would say it would help you lose weight. [/s]\\
% & how can anybody get rich, like you can get your self from your boss in bed? you are more likely to get your\\
% & money! you'll get some extra money!! [/s]\\
% &can anyone explain this riddle for men? \_UNK - its as simple as men ' ' women --)? what are women doing \\
% & about it in your opinion? [/s]\\
% &\_UNK of course a theory without the scientific research theory is this is? is it a \_UNK ' theory of \\
% &evolution, evolution? what? well, if you are looking for a good answer. [/s]\\
% &what foods available mainly by foods with food that's the fruit of the food? well soy milk contains vitamin d \\
% & in it milk vitamin c - ( and all the \_UNK ) contains lactose. [/s]\\
% &what are some similarities to globalization development? it's important to provide some information about a \\
% &particular subject and some links to an interesting and interesting , detailed description. [/s]\\
& \tabitem is anyone willing to donate plasma if you are allergic to cancer or anything else? probably you can. i've never\\
& done any thing but it is only that dangerous to kill bacteria. i have heard that it doesn't have any effect on\\ &your immune system. [/s]\\
% &does all sorts of stuff really make i get a good answer without just asking me out a lot of the questions on here \\
% &are some good sites to see here in replying and answers the questions that a few questions were asked to be \\
% &answered [/s]\\
\bottomrule
\end{tabular}
\end{center}
\caption{Generated Sentences on Yahoo Dataset.}
\label{table:results:sentences}
\end{table*}
